Detecting and Restoring Non-Standard Hands in Stable Diffusion Generated Images

We introduce a pipeline to address anatomical inaccuracies in Stable Diffusion generated hand images. The initial step involves constructing a specialized dataset, focusing on hand anomalies, to train our models effectively. A finetuned detection model is pivotal for precise identification of these anomalies, ensuring targeted correction. Body pose estimation aids in understanding hand orientation and positioning, crucial for accurate anomaly correction. The integration of ControlNet and InstructPix2Pix facilitates sophisticated inpainting and pixel-level transformation, respectively. This dual approach allows for high-fidelity image adjustments. This comprehensive approach ensures the generation of images with anatomically accurate hands, closely resembling real-world appearances. Our experimental results demonstrate the pipeline's efficacy in enhancing hand image realism in Stable Diffusion outputs. We provide an online demo at https://fixhand.yiqun.io

==> 2-relatedWork.tex <==
\section{Related Work}\label{sec:related}



==> 4-experiment.tex <==
\section{Experiment}\label{sec:experiment}

==> O-1-introduction.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[height=5.6cm]{images/introduction/non-standard-hand.png}
    \caption{A compilation of images with non-standard hand anomalies, highlighting the varied manifestations of the issue.}
    \label{fig:intro-non-standard}
\end{figure*}

\chapter{Introduction}

As the frontiers of artificial intelligence expand, the Stable Diffusion \cite{2022_ldm} model emerges as a formidable contender in the generation of human images. Its superior capability in crafting human likenesses, especially in real-time applications such as gaming or augmented reality, makes it an invaluable asset. However, we observe that the model frequently falters in generating hand images, leading to what we term as non-standard hand. As illustrated in \autoref{fig:intro-non-standard}, a non-standard hand can exhibit various anomalies such as missing fingers, an incorrect number of fingers, disproportionate size, or incorrect hand structure. Such inconsistencies, albeit subtle, can significantly compromise the overall realism and authenticity of the generated images.

\begin{figure}[!h]
    \centering
    \includegraphics[width=1\textwidth]{images/introduction/non-standard-hand.png}
    \caption{Some images with non-standard hand.}
    \label{fig:intro-non-standard}
\end{figure}

The phenomenon of the \textit{uncanny valley}\cite{mori1970bukimi} suggests that when humanoid objects appear almost, but not exactly, like real human beings, it elicits feelings of eeriness and discomfort among human observers. In the context of Stable Diffusion's generation of hand images, non-standard hands risk plunging generated figures into this uncanny valley. Furthermore, in applications like augmented reality (AR), virtual reality (VR) and gaming, where immersion and realism are paramount, such irregularities can become particularly jarring for users. The disruption caused by these non-standard hands can hinder the user experience, limiting the full potential of these technologies. Ensuring accurate hand depiction is thus not only about aesthetics but also about the usability and user satisfaction in dynamic virtual environments.

Besides Stable Diffusion, other image generative models such as Variational Autoencoders (VAEs) \cite{kingma2013auto} and Generative Adversarial Networks (GANs) \cite{goodfellow2014generative} also exist. However, compared to the adversarial training required by GANs or the variational posterior needed by VAEs, the predominant advantage of the Diffusion model lies in its simplicity of training. Leveraging the architecture of UNet \cite{ronneberger2015u} from the domain of image segmentation, the Stable Diffusion model boasts a stable training loss and exceptional performance. We perceive Stable Diffusion to be of greater practical value. This inherent strength of Stable Diffusion has driven our focus towards addressing the non-standard hand anomalies specifically within Stable Diffusion.

We conjecture that Stable Diffusion tends to generate non-standard hands because of its inherent challenges in capturing spatial positioning, proportions, and detailed intricacies, particularly in 3D to 2D representations. We draw insights from \cite{ramesh2022hierarchical}, DallE2, another diffusion model. It has also shown limitations in handling spatial positioning and proportions, as evident from \autoref{fig:intro-dalle-1}, one input (red cube on top, blue cube on bottom) gets a lot of confusing outputs. In addition, \autoref{fig:intro-dalle-2} shows the model's challenges in capturing intricate details within complex scenes. A significant contributor to this limitation might be the Contrastive Language-Image Pre-Training (CLIP) architecture they employed. In the CLIP training phase, the model predominantly learns from holistic image descriptions, often overlooking fine details such as those of hands. Thus, the nuances of hand articulations might elude these models. Another plausible explanation for this observed anomaly in hand generation could be the inherent complexity of hands as a 3D structure. Even slight alterations, such as rotations, can introduce significant variances when represented in a 2D image. Since Stable Diffusion primarily trains on 2D representations, it might be challenged in assimilating the comprehensive 3D intricacies of hands. This insufficiency potentially results in detailed inaccuracies when generating novel hand images.

\begin{figure}[!h]
	\centering
	\subfigure[Confused spatial positioning.]{
		\begin{minipage}[b]{0.45\textwidth}
			\includegraphics[height=5cm,keepaspectratio]{images/introduction/dalle-1.png} 
		\end{minipage}
		\label{fig:intro-dalle-1}
	}
    \subfigure[Complex scene.]{
		\begin{minipage}[b]{0.45\textwidth}
			\includegraphics[height=5cm,keepaspectratio]{images/introduction/dalle-2.png} 
		\end{minipage}
		\label{fig:intro-dalle-2}
	}
    \caption{Illustrations from Ramesh \etal \cite{ramesh2022hierarchical}.}
\end{figure}


Despite the evident necessity to resolve this challenge, there's a conspicuous scarcity of comprehensive research in this realm. To bridge this gap, our work introduces a systematic methodology that first detects the non-standard hand and then restores them to resemble real-world hand images, which we denote as standard hand. Our proposed pipeline seamlessly integrates detection and restoration. The process kicks off with the detection phase, which is engineered to identify both standard and non-standard hand types in images using bounding boxes. Harnessing a dedicated dataset and leveraging the prowess of the YOLOv8 model \cite{yolov8}, our method achieves commendable precision in this phase, example of detection phase is illustrated in \autoref{fig:intro-detection}.

\begin{figure}[!h]
	\centering
	\subfigure[Image with both standard and non-standard-hand.]{
		\begin{minipage}[b]{0.31\textwidth}
			\includegraphics[height=5cm,keepaspectratio]{images/introduction/detection-a.png} 
		\end{minipage}
	}
    \subfigure[Result of detection.]{
		\begin{minipage}[b]{0.31\textwidth}
			\includegraphics[height=5cm,keepaspectratio]{images/introduction/detection-b.png} 
		\end{minipage}
	}
    \subfigure[Mask of only non-standard hand.]{
		\begin{minipage}[b]{0.31\textwidth}
			\includegraphics[height=5cm,keepaspectratio]{images/introduction/detection-c.png} 
		\end{minipage}
	}

    \caption{Example of detection.}
    \label{fig:intro-detection}
\end{figure}

With the anomalies detected, our approach transitions to the restoration phase. Here, our pipeline meticulously follows a sequence of steps: \textit{Body Pose Estimation}, which leverages Google's MediaPipe \cite{mediapipe} to establish hand orientation; \textit{Control Image Generation}, a key step that guides the subsequent restoration by producing instructive images for the Stable Diffusion model; \textit{ControlNet Inpainting}, wherein the image undergoes initial restoration aided by the Control Image; and, finally, \textit{IP2P Inpainting}, a finishing touch to impart the generated hand images with life-like textures and authentic appearances. The pipeline overview is shown in \autoref{fig:intro-pipeline}.
\begin{figure}[!h]
	\centering
	\subfigure[Images with non-standard-hand.]{
		\begin{minipage}[b]{0.31\textwidth}
			\includegraphics[height=5cm,keepaspectratio]{images/introduction/02-redrawn.png} 
		\end{minipage}
	}
    \subfigure[Zoom in of non-standard-hand.]{
		\begin{minipage}[b]{0.31\textwidth}
			\includegraphics[height=5cm,keepaspectratio]{images/introduction/02-redrawn-zoom-in.png} 
		\end{minipage}
	}
    \subfigure[Result of non-standard hand detection.]{
		\begin{minipage}[b]{0.31\textwidth}
			\includegraphics[height=5cm,keepaspectratio]{images/introduction/02-redrawn-bbox.png} 
		\end{minipage}
	}

    \subfigure[Control image visualization.]{
		\begin{minipage}[b]{0.31\textwidth}
			\includegraphics[height=5cm,keepaspectratio]{images/introduction/02-control-a.png} 
		\end{minipage}
	}
    \subfigure[Zoom in of control image visualization.]{
		\begin{minipage}[b]{0.31\textwidth}
			\includegraphics[height=5cm,keepaspectratio]{images/introduction/02-control-a-zoom-in.png} 
		\end{minipage}
	}
    \subfigure[ControlNet inpainting.]{
		\begin{minipage}[b]{0.31\textwidth}
			\includegraphics[height=5cm,keepaspectratio]{images/introduction/02-controlnet.png} 
		\end{minipage}
	}


    \subfigure[Zoom in of controlNet inpainting.]{
		\begin{minipage}[b]{0.31\textwidth}
			\includegraphics[height=5cm,keepaspectratio]{images/introduction/02-controlnet-zoom-in.png} 
		\end{minipage}
	}
    \subfigure[IP2P inpainting.]{
		\begin{minipage}[b]{0.31\textwidth}
			\includegraphics[height=5cm,keepaspectratio]{images/introduction/02-ip2p.png} 
		\end{minipage}
	}
    \subfigure[Zoom in of IP2P inpainting.]{
		\begin{minipage}[b]{0.31\textwidth}
			\includegraphics[height=5cm,keepaspectratio]{images/introduction/02-ip2p-zoom-in.png} 
		\end{minipage}
	}
    \caption{Pipeline overview.}
    \label{fig:intro-pipeline}
\end{figure}

After our experiments in \autoref{chap:experiment}, our pipeline has achieved good results. Our fine-tuned YOLOv8 model impressively distinguishes between non-standard hand and standard hand. Moreover, during the restoration phase, our methodology demonstrably and gracefully transforms the non-standard hand to closely match the standard variant.

In order to bridge the gap between advanced research methodologies and end-user accessibility, we have developed an interactive web application that encapsulates our novel hand-restoration approach. We provide a comprehensive guide to this software in \autoref{chap:software}. This user-friendly platform allows users to swiftly upload images containing non-standard hands and, within moments, receive immediate restoration feedback. Our intention behind this design is to ensure that our sophisticated methods can be easily leveraged, providing both enthusiasts and professionals a firsthand experience of the transformative power of our technology.

Through this report, we anticipate offering a robust solution that amplifies the quality of images generated by Stable Diffusion, with a special focus on enhancing the representation of hands, one of the most expressive parts of the human body. The main contributions are as follows:


\begin{enumerate}
    \item We curated a new dataset by leveraging the HaGRID dataset \cite{hagrid}. The dataset has a lot of labeled standard and non-standard hands, preparing for the next standard and non-standard hand to be detected.
    
    \item With the objective of achieving precise detection and classification capabilities, the YOLOv8 model was fine-tuned. This enhanced version exhibits a remarkable prowess in distinguishing between standard and non-standard hand images.
    
    \item Our work introduces a dedicated pipeline aimed at non-standard hand restoration. This pipeline, uniquely crafted, ensures meticulous attention to the restoration process, consequently refining the final image quality.
    
    \item The efficacy of our restoration methodology has been solidified through rigorous experiments. Our results corroborate that not only is our approach effective within the Stable Diffusion generated images, but it also exhibits commendable restoration capabilities on images with diverse styles.
    
    \item To bridge the divide between complex computational methodologies and user accessibility, we've launched an interactive web application. This platform embodies our entire restoration process, enabling users to witness and experience the transformational prowess of our technology in real-time.
\end{enumerate}



==> O-2-relatedWork.tex <==
\chapter{Literature Review}\label{chap:literaturerwview}

\section{Detection}

\subsection{Grounding DINO}
% Openset detection
Object detection can be classified as closed-set object detection and open-set object detection.
In closed-set object detection, the model is trained on a specific set of object classes and is expected to detect and classify objects only from these classes in the test data. It assumes that all possible object categories are included in the training set. Objects that don't belong to any of the trained classes might be misclassified into one of the known classes or simply ignored.
In contrast, open-set object detection can handle the detection of unknown or unseen object classes, which were not present in the training data. When faced with objects from these novel classes in the test data, the model is expected to recognize that they don't belong to any of the classes it was trained on and ideally classify them as unknown or assign a low confidence score. Open-set object detection is more suitable for real-world scenarios where the variety of objects encountered can be vast and unpredictable.

% DINO
DINO is a DEtection TRansformer(DETR~\cite{DETR})-like model that harnesses end-to-end Transformer-based detection. DINO~\cite{dino} integrates advanced techniques such as contrastive de-noising and achieves unprecedented performance on the COCO object detection benchmark. Nonetheless, DINO~\cite{dino} targets closed-set detection, and its capacity to adapt to unseen classes is constrained by predefined category limitations.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{images/dino_and_groundingdino.pdf}
    \caption{Comparison between DINO and Grounding DINO. The modifications are marked in blue. Best viewed in color. This figure is from~\cite{groundingDINO}.}
    \label{fig:dino_and_groundingdino}
    % \vspace{-0.8cm}
\end{figure*}

% Grounding DINO contribution
Grounding DINO~\cite{groundingDINO} is an open-set detector based on DINO~\cite{dino}, which extends the closed-set detector DINO by performing vision-language modality fusion at multiple phases, including a feature enhancer, a language-guided query selection module, and a cross-modality decoder. Such a deep fusion strategy effectively improves open-set object detection. A comparison between DINO and Grounding DINO can be found in Fig~\ref{fig:dino_and_groundingdino}.

Grounding DINO's architecture has the following advantages. 
First, Grounding DINO is Transformer-based, which aligns with established language models, ensuring simultaneous and efficient processing of both visual and linguistic data. This alignment contributes to the integration of cross-modal features throughout the pipeline. 
Second, Transformer-based detectors have consistently showcased adeptness in employing large-scale datasets. 
Lastly, DINO is an end-to-end architecture, eliminating the necessity for handcrafted modules like Non-Maximum Suppression (NMS).

Grounding DINO proposes to fuse features across the various phases of detection. While prior models selectively fuse features, the authors found that a comprehensive fusion, early in the detection pipeline, is more beneficial for open-set detection, especially when both image and text inputs are available from the start. These fusion methods encompass a feature enhancer mechanism and a language-guided query selection, ensuring a more robust detection performance.

The experiments not only measure the model's efficacy in detection novel categories but also evaluate its performance on Referring Expression Comprehension (REC) datasets. Such datasets involve objects described with attributes, offering another layer of complexity to the detection process.
Experiments show Grounding DINO's superiority over its contemporaries. Impressively, without any training data from COCO, it achieved a 52.5 AP on the COCO minival. Furthermore, it set a new benchmark in the ODinW zero-shot category with a 26.1 mean AP. 

However, despite these notable achievements, Grounding DINO has its limitations. This model is not suitable for segmentation tasks. Additionally, the training data used for Grounding DINO is relatively smaller than the most extensive GLIP model, potentially hindering its maximum performance.


\subsection{Segment Anything}

\begin{figure*}[t]\centering
\includegraphics[width=0.99\linewidth]{images/sam.pdf}
\caption{Segment Anything Model~\cite{sam} overview. An image encoder extracts the image embedding which can be queried by various input prompts to retrieve object masks. This figure is from~\cite{sam}.}
\label{fig:model_diagram}
\end{figure*}

Segment Anything~\cite{sam} tries to employ the cutting-edge capabilities observed in foundation models for natural language processing (NLP) in the image segmentation task.

In the recent surge of NLP advancements, large-scale models pretrained on web-scale datasets, often dubbed as \textit{foundation models} \cite{bommasani2021opportunities}, have showcased robust zero-shot and few-shot generalization capabilities. These models are able to generate appropriate textual responses even for tasks unseen during their training.

Drawing inspiration from this, Segment Anything is proposed as a \textit{foundation model} for image segmentation. The authors define a general promptable segmentation task, design a promptable model and pre-train it on a broad dataset to solve a range of downstream segmentation tasks on new data distributions using prompt engineering. On the training, it supervises mask prediction through the linear combination of focal loss \cite{lin2017focal} and dice loss \cite{milletari2016v} as employed in \cite{carion2020end}. The main contributions include:

\begin{itemize}
    \item \textbf{Promptable Segmentation Task (PST):} The authors introduced a new task, where a valid segmentation mask is expected to return given any segmentation prompt. A prompt specifies the spatial or text clue to objects in an image. Even when an ambiguous prompt is provided, which can refer to multiple objects in an image, a reasonable mask for at least one of them will return. 
    This task not only serves as a pre-training objective but also can solve various downstream segmentation problems via prompt engineering.
    
    \item \textbf{Segment Anything Model (SAM):} SAM was designed to efficiently handle the PST. It consists of an image encoder, a prompt encoder, and a mask decoder. By integrating these components, SAM can handle flexible prompts and produce segmentation masks in real-time, which is pivotal for interactive applications. To handle the prompt ambiguity, SAM supports the prediction of multiple plausible masks for a single prompt.
    
    \item \textbf{SA-1B Dataset:} Recognizing the scarcity of large-scale segmentation datasets, the authors build an innovative \textit{data engine}, a system where SAM was involved and developed in an iterative data annotation loop. The final dataset SA-1B contains over 1 billion masks across 11 million images. 
\end{itemize}

Through extensive experiments, SAM exhibited remarkable performance across different segmentation tasks under zero-shot transfer scenarios using prompt engineering.

% In the pioneering work titled "Segment Anything", the authors present an ambitious endeavor to bridge the gap between traditional image segmentation and the cutting-edge capabilities observed in foundation models for natural language processing (NLP). In the recent surge of NLP advancements, large-scale pre-trained models, often dubbed as "foundation models", have showcased unprecedented abilities in both zero-shot and few-shot generalizations. These models, when prompted with hand-crafted textual inputs, exhibit commendable competencies in generating appropriate textual responses even for tasks unseen during their training.

% Drawing inspiration from this, the authors of "Segment Anything" envisioned an analogous feat for image segmentation. They introduced a new task, model, and dataset to foster a similar paradigm shift in the realm of computer vision. Their principal contributions include:

% \begin{itemize}
%     \item \textbf{Promptable Segmentation Task (PST):} Leveraging the power of "prompting", they devised a task where a model is expected to return a valid segmentation mask in response to any segmentation prompt. This could range from spatial markers to textual cues, pinpointing objects within an image. Their task not only serves as a pre-training objective but is also adapted to cater to diverse downstream segmentation problems via apt prompt engineering.
    
%     \item \textbf{Segment Anything Model (SAM):} SAM was designed to efficiently handle the PST. It consists of an image encoder, a prompt encoder, and a mask decoder. By integrating these components, SAM can nimbly handle flexible prompts and produce segmentation masks in real-time, a pivotal attribute for interactive applications. To address inherent ambiguities in images, SAM was engineered to predict multiple plausible masks for a single prompt.
    
%     \item \textbf{SA-1B Dataset:} Recognizing the scarcity of large-scale segmentation datasets, the authors introduced SA-1B, a behemoth dataset housing over 1 billion masks across 11 million images. This dataset, unparalleled in its scale and diversity, was created using their innovative "data engine", a system where SAM was intrinsically involved in an iterative data collection and refinement loop.
% \end{itemize}

% Through extensive experiments, SAM exhibited remarkable results across a myriad of segmentation tasks under zero-shot transfer scenarios using prompt engineering. Despite its promising achievements, the authors acknowledged areas for further enhancements.

\subsection{Grounded-Segment-Anything}

In the quest for developing AI models that can robustly detect and delineate objects in images based on textual inputs, a prominent effort known as the Grounded-Segment-Anything (GSA) \cite{GSA} was introduced. This innovative approach envisaged the integration of two potent AI models, namely, \textit{Grounding DINO} and \textit{Segment Anything}. The main ambition behind GSA was to offer a mechanism capable of both detecting and segmenting any object by simply employing text as an input descriptor. At its heart, the motivation behind GSA's creation stems from an aspiration to amalgamate the unique strengths of diverse AI models, thus constructing an authoritative pipeline to tackle multifaceted challenges.


\subsection{YOLO}

\textit{You Only Look Once: Unified, Real-Time Object Detection} \cite{redmon2016you} has markedly reshaped the landscape of object detection in computer vision. Their proposed framework, YOLO, is emblematic for its innovative approach to the problem at hand. 

Historically, object detection methodologies have largely been rooted in adapting classifiers for detection. Traditional systems, such as the Deformable Parts Models (DPM) \cite{felzenszwalb2009object}, employ a sliding window approach, which necessitates running the classifier at uniformly spaced locations across the entirety of the image. More contemporary techniques, such as R-CNN \cite{girshick2014rich}, pivot to a two-stage mechanism—initially generating potential bounding boxes via region proposal methods, followed by deploying a classifier on these suggested regions. An ensuing post-processing phase refines these bounding boxes, eradicates duplicative detections, and recalibrates box scores based on the surrounding objects in the scene. However, these intricate pipelines bear inherent drawbacks: they are computationally intensive, not entirely optimized, and each component mandates independent training.

\begin{figure}[!h]
    \centering
    \includegraphics[width=1\textwidth]{images/relatedWork/yolo-v1-2.png}
    \caption{The YOLO architecture. The detection architecture we've designed comprises $24$ convolutional layers, succeeded by $2$ fully connected layers. Interspersed $1 \times 1$ convolutional layers serve to diminish the feature space derived from the layers before them. The initial training of the convolutional layers takes place on the ImageNet classification task with a resolution halved ($224 times 224$ input image). Post this, the resolution is doubled for the detection phase.}
    \label{fig:relatedwork-yolo-v1-2}
\end{figure}

In stark contrast, YOLO offers a refreshing perspective. It reconceptualizes object detection as a singular regression problem, transitioning directly from image pixels to bounding box coordinates and the affiliated class probabilities. This conceptual shift is underpinned by a significant architectural transformation. YOLO's unified architecture ensures that a single convolutional network concurrently predicts multiple bounding boxes and the associated class probabilities for those boxes. One of the seminal achievements of this approach is the holistic view it maintains during both the training and testing phases. By processing the complete image, YOLO intrinsically garners rich contextual insights, bolstering its ability to discern objects from backgrounds with heightened accuracy.

\begin{figure}[!h]
    \centering
    \includegraphics[width=1\textwidth]{images/relatedWork/yolo-v1-1.png}
    \caption{The approach YOLO employ models detection as a regression challenge. We segment the image into an $S \times S$ grid. For each segment, the system forecasts $B$ bounding boxes along with their respective confidences and C probabilities for each class. The outcome of these predictions is represented as an $S \times S \times (5B + C)$ tensor.}
    \label{fig:relatedwork-yolo-v1-1}
\end{figure}

The merits of YOLO are manifold. Foremost, its efficiency metrics are unparalleled. YOLO's streamlined architecture eliminates the need for a multifaceted pipeline. As such, the neural network can simply be executed on a new image during testing, enabling real-time detections. This swiftness is empirically substantiated—the base YOLO model processes images at an astonishing 45 frames per second, with the Fast YOLO variant reaching up to 155 frames per second. Moreover, the YOLO framework displays a laudable balance between speed and precision, often surpassing the mean average precision of its contemporaneous real-time counterparts.

Equally significant is YOLO's adaptability and generalizability. This versatility is particularly evident when it is subjected to domain variations. For instance, models trained on conventional natural images, when tested on diverse domains like artwork, have consistently demonstrated superior performance compared to erstwhile state-of-the-art models like DPM and R-CNN.

Nevertheless, no model is without its imperfections. Despite its groundbreaking contributions, YOLO isn't immune to certain challenges. Specifically, while it excels in rapidly identifying objects within images, it occasionally grapples with exact localization, particularly concerning smaller objects.

In conclusion, the YOLO framework represents a quantum leap in the realm of real-time object detection. By unifying the model structure and espousing a regression-based approach, it not only accelerates detection speeds but also sets a benchmark in adaptability across varied domains.


\subsection{YOLOv8}

\textit{Ultralytics} introduced YOLOv8 \cite{yolov8} as the successor to YOLOv5, amplifying the object detection capabilities and delivering a state-of-the-art performance in a variety of computer vision tasks. Launched in January 2023, YOLOv8 embodies a convergence of advanced features that push the boundaries of speed, accuracy, and adaptability. Distinct from its predecessors, the YOLOv8's architecture and operational paradigm are rooted in meticulous innovations and are inspired by cutting-edge research. As you can see in \autoref{fig:relatedwork-yolo-v8-1}, YOLOv8's performance is significantly better than its predecessor.

\begin{figure}[!h]
    \centering
    \includegraphics[width=1\textwidth]{images/relatedWork/yolo-v8-1.png}
    \caption{YOLO comparison.}
    \label{fig:relatedwork-yolo-v8-1}
\end{figure}

Diving into the nuances of the YOLOv8 model:
\begin{itemize}
    \item The core of YOLOv8 is a detection network that provides multiple resolutions. To cater to a spectrum of deployment scenarios, YOLOv8 offers model variants across various scales, such as N, S, M, L and X, like YOLOv5 \cite{yolov5}. These variants can balance the computing speed and model performance.
    
    \item In terms of architectural refinement, YOLOv8 borrows inspiration from the YOLOv7's \cite{wang2023yolov7} ELAN design philosophy. The backbone and the Neck segment of the model underwent pivotal transformations. Specifically, the C3 structure from YOLOv5 was evolved into a richer gradient flow, known as the C2f structure. This meticulous restructuring allows for more tailored channel adjustments across different scaled models, leading to substantial performance boosts. It's worth noting, however, that certain operations within the C2f module, such as the Split operation, might introduce challenges for deployment on specific hardware platforms.
    
    \item One of the significant overhauls in YOLOv8 lies in the model's Head section. Departing from the traditional Anchor-Based approach prevalent in YOLOv5, YOLOv8 adopts an Anchor-Free paradigm. Additionally, the classification and detection heads are decoupled, streamlining the detection process.
    
    \item On the loss computation front, YOLOv8 incorporates the TaskAlignedAssigner for positive sample allocation, complemented by the Distribution Focal Loss. These refinements ensure more robust gradient updates during training, facilitating better model convergence.
    
    \item Training data augmentation has been enhanced by borrowing strategies from YOLOX, especially the technique of deactivating the Mosaic augmentation in the last 10 epochs, a measure that has proven effective in elevating model accuracy.
\end{itemize}

In essence, YOLOv8, while echoing the legacy of its YOLO lineage, takes a pragmatic turn towards engineering optimization. It melds together insights from recent breakthroughs like YOLOX \cite{ge2021yolox}, YOLOv6 \cite{li2022yolov6}, YOLOv7, and PPYOLOE. While its innovations might appear incremental, they culminate in a formidable framework that stands as a benchmark in real-time object detection and segmentation.

\section{Pose Estimation}

\subsection{AlphaPose}

In recent times, whole-body multi-person pose estimation and tracking have emerged as pressing challenges in the realm of computer vision. Before that, there have been some top-down \cite{pishchulin2012articulated, gkioxari2014using} frameworks and bottom-up \cite{chen2015parsing, pishchulin2016deepcut, insafutdinov2016deepercut} frameworks. A response to this need has been offered through the introduction of AlphaPose, a system designed to efficiently estimate and track whole-body poses in real-time, proposed by \textit{AlphaPose: Whole-Body Regional Multi-Person Pose Estimation and Tracking in Real-Time} \cite{alphapose} is illustrated in \autoref{fig:related-alphapose-2}. Differentiating itself from conventional body-only pose estimation, AlphaPose aims to capture subtle human actions by focusing on the entirety of the human figure: face, body, hand, and foot.

The crux of the AlphaPose system is built upon several innovative techniques. The first, Symmetric Integral Keypoint Regression (SIKR), ensures rapid yet precise localization. Another noteworthy method, Parametric Pose Non-Maximum-Suppression (P-NMS), is employed to diminish redundant human detections. This is achieved through the implementation of a novel pose distance metric that effectively gauges pose similarity. To synergize pose estimation and tracking, the Pose Aware Identity Embedding technique is utilized. This combined approach relies on a person re-id branch integrated within the pose estimator, thereby streamlining the real-time estimation and tracking processes.

Notably, the research identifies the shortcomings of the widely accepted heatmap representation, especially when used to localize keypoints across diverse body parts. The discrete nature of heatmap representation often leads to quantization errors which impede accurate estimation of intricate keypoints like those on hands and faces. Unlike the previous use more sub-networks for hand and face estimation \cite{cao2017realtime} and use ROI-Align to enlarge the feature map \cite{jin2020whole}, AlphaPose proposes a symmetric integral keypoints regression approach, presenting a solution that combines the precision of heatmap representation while also eliminating its inherent errors.

\begin{figure}[!h]
    \centering
    \includegraphics[width=1\textwidth]{images/relatedWork/alphapose-1.png}
    \caption{Errors in quantization due to the heatmap are indicated by the green and blue lines. By employing our symmetric integral keypoints regression, denoted by the pink line, AlphaPose can effectively address the localization discrepancy.}
    \label{fig:related-alphapose-1}
\end{figure}

Acknowledging the scarcity of training data for full-body pose estimation, the authors have introduced the Halpe dataset, offering additional essential joints that were previously unavailable. Augmenting this, they have incorporated a Multi-Domain Knowledge Distillation technique and an innovative Part-Guided Proposal Generator (PGPG) to simulate the generation of human bounding boxes, thus producing an ample set of training data.

AlphaPose's inception has been met with significant recognition in the research community, with its library already receiving substantial attention on platforms like GitHub. Moreover, its comprehensive nature is not limited to pose estimation and tracking; it also holds potential for extensions into 3D keypoints and mesh inclusion, signaling promising directions for future research endeavors.

\begin{figure}[!h]
    \centering
    \includegraphics[width=1\textwidth]{images/relatedWork/alphapose-2.png}
    \caption{Illustration of AlphaPose's full-body pose estimation and tracking framework.}
    \label{fig:related-alphapose-2}
\end{figure}

In conclusion, the AlphaPose system represents a leap forward in the pursuit of accurate and efficient whole-body multi-person pose estimation and tracking. Its innovative methodologies, coupled with the provision of a new dataset and optimized standard library, make it an invaluable tool for both researchers and practitioners in the computer vision domain.

\subsection{ViTPose}

In the realm of computer vision, the application of Vision Transformers (ViTs) \cite{dosovitskiy2020image} has seen significant success across a myriad of tasks, especially in image classification. Yet, their capacity for human pose estimation, a task fundamentally centered on localizing human anatomical keypoints, remains somewhat unexplored. The paper titled \textit{ViTPose: Simple Vision Transformer Baselines for Human Pose Estimation} \cite{xu2022vitpose} dives deep into this very question, and presents an innovative application of ViTs to this challenging domain. Its architecture is illustrated in \autoref{fig:related-vit-1}.

Traditional methods for pose estimation primarily hinge on Convolutional Neural Networks (CNNs) \cite{lecun1998gradient}, exploiting their spatial hierarchies to detect and map intricate human structures \cite{li2021pose, li2021tokenpose, yang2021transpose}. However, as evidenced in recent years, ViTs exhibit a noteworthy capability in processing visual data, motivating their exploration in tasks beyond mere classification. What distinguishes ViTPose from prior works is its pristine reliance on plain vision transformers. It avoids the convolution-heavy architectures or intricate designs typically seen in its predecessors.

\begin{figure}[!h]
    \centering
    \includegraphics[width=1\textwidth]{images/relatedWork/vit-1.png}
    \caption{Architecture of ViTPose.}
    \label{fig:related-vit-1}
\end{figure}

The core of ViTPose rests on using plain and non-hierarchical vision transformers as backbones to extract salient features from given human instances. These backbones are initialized with pre-training schemes using masked image modeling pretext tasks, ensuring a robust start for downstream pose estimation tasks. Upon feature extraction, a concise decoder further processes the features. This involves upscaling the feature maps and subsequently regressing the heatmaps in relation to the keypoints. Remarkably, despite its structural simplicity, ViTPose sets a new benchmark with a performance of 80.9 AP on the challenging MS COCO Keypoint test-dev dataset.

The ViTPose framework brings forth four salient strengths:

\begin{enumerate}

\item \textbf{Simplicity:} With the powerful feature representation capability of ViTs, the ViTPose model enjoys an elegant design. The encoder entails stacking plain transformer layers, and the decoder can be further distilled to an up-sampling layer followed by a convolutional prediction layer, with a negligible performance decrement.

\item \textbf{Scalability:} The inherent modularity of ViTPose allows it to easily adapt to different computational requirements. By varying the number of transformer layers or adjusting the feature dimensions, one can easily strike a balance between performance and computational costs.

\item \textbf{Flexibility:} ViTPose showcases adaptability across various training paradigms. It can cater to different input resolutions, can be adapted to multiple pose datasets with minimal modifications, and still delivers top-tier performance even when trained on smaller datasets or under constrained settings.

\item \textbf{Transferability:} The knowledge encapsulated within larger ViTPose models can be seamlessly transferred to their smaller counterparts using an innovative knowledge token, demonstrating the model's inherent capability for knowledge distillation.

\end{enumerate}

In summation, ViTPose epitomizes a paradigm shift in human pose estimation. By showcasing that simple and plain vision transformer architectures can not only match but potentially surpass the capabilities of their convolution-heavy counterparts, this work provides a promising direction for the evolution of pose estimation techniques. Moreover, the traits of simplicity, scalability, flexibility, and transferability exhibited by ViTPose illuminate the vast potential of vision transformers in broader computer vision applications.


\subsection{BlazePose}

Meidapipe \cite{mediapipe} is a machine learning kit from Google, which contains many solutions. It also includes a model for body pose estimation, also known as solution Pose Landmark Detection, which is BlazePose \cite{bazarevsky2020blazepose}, from the paper \textit{BlazePose: On-device Real-time Body Pose tracking}

BlazePose introduces a lightweight convolutional neural network architecture that efficiently produces 33 body keypoints for a single person is illustrated in \autoref{fig:related-blazepose-1}. Remarkably, this system operates at over 30 frames per second even on modest hardware, such as a Pixel 2 phone, showcasing its applicability in real-time scenarios like fitness tracking and sign language recognition.

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.4\textwidth]{images/relatedWork/BlazePose-1.png}
    \caption{BlazePose 33 keypoint topology.}
    \label{fig:related-blazepose-1}
\end{figure}

A pivotal challenge in human body pose estimation arises from the diverse range of human poses, the substantial degrees of freedom, and prevalent occlusions. While prior research has made noteworthy advancements in this domain, many existing approaches, particularly those generating heatmaps for each joint \cite{sun2019deep, kreiss2019pifpaf}, result in models too bulky for real-time mobile deployment. BlazePose confronts this issue head-on, achieving considerable acceleration of the model with minimal compromise on quality.

BlazePose departs from traditional heatmap-based techniques, which, despite their scalability, typically involve substantial computational overhead. Instead, it adopts a regression-based approach, aiming to predict mean coordinate values directly. This method, generally less computationally intensive, addresses the ambiguity often encountered in heatmap-based models. Building on the foundation laid by Newell \etal \cite{newell2016stacked}. with the stacked hourglass architecture, BlazePose employs an encoder-decoder network to initially predict heatmaps for all joints. This is followed by another encoder that regresses directly to the coordinates of all joints. A key innovation in BlazePose is the discardable heatmap branch during inference, significantly reducing the model's footprint and enabling its deployment on mobile platforms.

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.6\textwidth]{images/relatedWork/BlazePose-2.png}
    \caption{BlazePose results on yoga and fitness poses.}
    \label{fig:related-blazepose-2}
\end{figure}


\section{Inpainting}

\input{diff_model_foundation}
\input{rel_sd}
\input{rel_control}
\input{rel_ip2p}

==> O-2-relatedWork/rel_control.tex <==
\subsection{ControlNet}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{images/controlnet_example.pdf}
    \caption{Controlling Stable Diffusion with Customized Conditions: ControlNet facilitates the inclusion of conditions like Canny edges (top), human pose (bottom), among others, to dictate the image generation trajectory of expansive pre-trained diffusion models. While the default prompt "a high-quality, detailed, and professional image" is utilized, users have the latitude to furnish specific prompts such as "chef in kitchen" to further steer the generation process. The image is adapted from~\cite{2023_controlnet}.}
    \label{fig:controlnet_example}
\end{figure}

ControlNet~\cite{2023_controlnet} aims to incorporate spatially localized conditioning controls into a broad array of pretrained diffusion models. The primary objective of this work is to provide end-users with a means of introducing conditions, such as Canny edges and human poses, to steer the generation of images from diffusion models. Examples are shown in~\autoref{fig:controlnet_example}. 

As~\autoref{fig:controlnet_architecture} shows about the architecture, the model mainly adopts an encoder-decoder architecture and houses several blocks, comprising convolution layers and main blocks with ResNet layers~\cite{2016_he2016deep} and Vision Transformers (ViTs)~\cite{2022_vit_survey} primarily to handle text prompts encoded with CLIP~\cite{2021_clip_paper}. This structure is implemented at the encoder level and is computationally optimized to conserve GPU memory and reduce training time.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.6\linewidth]{images/controlnet_architecture.png}
    \caption{Our Stable Diffusion's U-net structure integrates with a ControlNet at the encoder sections and the central block. The fixed, gray blocks depict the configuration of Stable Diffusion V1.5 (identical to V2.1, as they both utilize the same U-net design). The modifiable blue sections, coupled with the pristine white zero convolution layers, are incorporated to form the ControlNet. For a visual representation, refer to the image sourced from~\cite{2023_controlnet}.}
    \label{fig:controlnet_architecture}
\end{figure}

The essence of ControlNet lies in its ability to lock a significant portion of the original diffusion model, with training only affecting a copy of certain blocks, thus allowing the coexistence of new learning with established backbones. This is enabled through a scheme called 'Zero Convolutions', wherein convolution layers have their weight and bias parameters initialized to zeroes, facilitating the gradual increase of trainable parameters without introducing harmful noise.

During training, the input image is first transformed into a feature space vector via an encoding network, following which the image diffusion algorithms are employed to predict the noise expected in the noisy image after a designated number of noise additions. Subsequent to operations like feature-space conditioning vector evaluation, a sequence of steps including prompt replacement and weighted mixings are undertaken to finally derive the model output.

The comprehensive demonstration suggests that integrating ControlNet into pretrained diffusion models significantly enhances their capabilities by enabling the incorporation of diverse conditions. This presents a pathway of potential benefits for a wider spectrum of applications in controlling image diffusion models.


==> O-2-relatedWork/rel_ip2p.tex <==
\subsection{InstructPix2Pix}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{images/ip2p_example.pdf}
    \caption{When presented with an image and a corresponding editing directive, \cite{2023_ip2p} efficiently executes the intended modification. Setting itself apart from other models, there's no need for intricate details concerning the source or target image. It accomplishes image alterations in just one forward sweep, negating the necessity for individual inversion or meticulous fine-tuning. The graphic is sourced from~\cite{2023_ip2p}.}
    \label{fig:ip2p_example}
\end{figure}


InstructPix2Pix ~\cite{2023_ip2p} offers a unique technique that facilitates image modifications based on textual directives. This research proposes an innovative combination of two pretrained entities: a linguistic model and an image dispersion model. This amalgamation aids in the creation of an extensive dataset filled with instances of image editing. Harnessing this dataset, the researchers then develop a conditional dispersion model adept at modifying real-world visual representations following given textual guidelines. Examples of this can be seen in \autoref{fig:ip2p_example}.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{images/ip2p_method.pdf}
    \caption{The methodology behind InstructPix2Pix involves two primary phases: the creation of an image editing dataset, followed by the training of a diffusion model leveraging this dataset. (a) Initially, a finely-tuned GPT-3 is deployed to generate editing instructions along with amended captions. (b) Subsequently, the synergy of StableDiffusion and Prompt-to-Prompt~\cite{2022_prompt_to_prompt} is harnessed to produce pairs of images corresponding to pairs of captions, thereby enabling the assembly of a dataset (c) encompassing over 450,000 training instances. (d) Finally, the InstructPix2Pix diffusion model is trained on the meticulously curated data to perform image edits based on the furnished instructions. During inference, \cite{2023_ip2p} proficiently generalizes to alter real images in accordance with human-crafted instructions. The image is adapted from~\cite{2023_ip2p}.}
    \label{fig:ip2p_method}
\end{figure}

\autoref{fig:ip2p_method} presents a visual explanation of InstructPix2Pix's approach. 

To synthesize the requisite training data, a language model is employed to generate plausible editing instructions given an image caption. The outcome of this process is a collection of "editing triplets": an input caption, an editing instruction, and the amended output caption. Subsequently, the language-based instructions are translated into actual image edits using a model known as Stable Diffusion, thereby yielding pairs of images that correspond to the textual editing instructions.

The text-to-image translation hinges on Stable Diffusion's capability to render multiple interpretations for a given text prompt. This is actualized by exploiting the diffusion model's ability to sample multiple plausible images for each text instruction. To ensure diversity in the generated samples, a degree of randomness is incorporated in the guidance weights during the training example generation process.

The paper delineates the training data generation method as follows:

\begin{itemize}
    \item An edit instruction and a modified caption are generated from an input caption using a fine-tuned large language model. Mathematically, this process can be expressed as: $(c_{I}, c_{T}, c_{I'}) = f_{LM}(c_{I})$, where $c_{I}$ denotes the input caption, $f_{LM}$ represents the language model, $c_{T}$ is the generated edit instruction, and $c_{I'}$ is the amended image caption.
    \item Pairs of images corresponding to the pre-edit and post-edit images are created using the editing instructions $c_{T}$ and the Stable Diffusion image model. This process can be articulated as: $(x, x') = f_{SD}(c_{I}, c_{T}, c_{I'})$, where $f_{SD}$ represents Stable Diffusion, and $x$, $x'$ are the pre-edit and post-edit images respectively.
\end{itemize}

Additionally, the authors introduce a form of diffusion guidance, where the guidance scales $s_{I}$ and $s_{T}$ can be modulated to control the congruence of the generated samples with the input image and the edit instruction, respectively. 

==> O-2-relatedWork/rel_sd.tex <==
\subsection{Stable Diffusion}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/sd_example.png}
    \caption{Examples of generated images using LDMs. The image is from~\cite{2022_ldm}. }
    \label{fig:sd_example}
\end{figure}

Stable diffusion is based on Latent Diffusion Models (LDMs), proposed in~\cite{2022_ldm}. It recognizes the commendable synthesis outcomes of denoising autoencoders and diffusion models (DMs), albeit at the expense of computational rigor and substantial GPU resources, rendering them challenging to manage.

Latent Diffusion Models are introduced as a remedy to the computational intricacy inherent in the training and sampling processes, thereby elevating efficiency and accessibility. The utilization of pretrained autoencoders in the latent space empowers the handling and control of data encapsulating more layers and complexity. The architecture is crafted to exhibit adaptability and flexibility, accommodating a variety of conditioning inputs.

Through experimental evaluations, the authors ascertain that LDMs outperform preceding models in tasks such as inpainting, semantic synthesis, and conventional image generation, all while markedly curtailing computational expenditures. This superior performance is ascribed to the LDMs' adeptness at retaining perceptually pertinent image information and eschewing irrelevant details, striking a balance between efficiency and high-fidelity image reconstruction. The validation of results is carried out employing quantitative metrics like FID (Fréchet Inception Distance) scores and PSNR (Peak Signal-to-Noise Ratio).

Driven by the aspiration to democratize advanced image synthesis models, this work endeavors to slash computational overhead without forsaking result quality. The authors posit that their method represents a stride towards surmounting the challenge of democratizing such models for the expansive research community.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{images/sd_architecture.png}
    \caption{Visualization of LDM's architecture. The image is from~\cite{2022_ldm}. }
    \label{fig:sd_architecture}
\end{figure}

The architecture of a Latent Diffusion Model is encapsulated by the expression:

\[
\mathbb{E}_{x \sim p} \left[ L_{\text{LDM}} \left( E (x), \theta, z_t, \tau_\theta \right) \right],
\]

where $E$ denotes the encoder, $\theta$ the decoder, $z_t$ the latent variable, and $L_{\text{LDM}}$ the learning objective function of the LDM. $x$ symbolizes the input data, and $\tau_\theta$ is a function projecting the conditioning input onto an intermediate layer of the UNet, thereby delineating the conditioning mechanism. \autoref{fig:sd_architecture} shows an illustration of the architecture. 



==> O-3-method.tex <==
\chapter{Method}\label{chap:method}

\section{Overview}

In the images generated by the Stable Diffusion, there exists a notable challenge: the frequent representation of hands that deviate from conventional appearance, termed as non-standard hand. Our methodology is structured to detect these anomalies and subsequently restore them to closely match real-world hand images, which we refer to standard hand.

Our approach can be broadly divided into two primary segments: detection and restoration. In the detection phase, we focus on identifying the presence of both standard and non-standard hands in images, marking them with bounding boxes.. This is achieved through the creation of a dedicated dataset and the fine-tuned detection model. Following the detection, the Restoring phase is engaged. Detection and restoration are combined into a pipeline, the steps are \textit{Non-standard Hand Detection}, \textit{Body Pose Estimation}, \textit{Control Image Generation}, \textit{ControlNet Inpainting} and \textit{IP2P Inpainting}, are illustrated in Fig1. Through the steps, our approach can restore non-standard hand. The subsequent sections delve deeper into the intricacies of each segment. The flowchart is displayed in \autoref{fig:flowchart}.

\begin{figure}[!h]
    \centering
    \includegraphics[width=1\textwidth]{images/flowchart.jpg}
    \caption{Flowchart of the whole pipeline: First we input the hand with non-standard hand, use YOLOv8 to label the bounding box of the non-standard hand, and make a mask, which we call the bounding box mask. The body skeleton will be calculated using MediaPipe, and based on the body skeleton, the template will be placed at the exact location of the non-standard hand, which is called the control image, and the template's bounding box and the bounding box mask together form the union mask. box mask together form the union mask. Use the control image and the prompt with the template description to repair the area covered by the union mask, and use IP2P and its prompt to further repair the texture to get the final output.}
    \label{fig:flowchart}
\end{figure}


\section{Non-Standard Hand Detection}

Non-standard hand detection phase is designed to locate the bounding boxes of all hands present within an image. Moreover, it categorizes these hands into two distinct categories: non-standard hand and standard hand.

\subsection{Non-Standard Hand Dataset} \label{section:method_detecting_database}

In order to achieve a precise localization and classification of hands within images, we need to create a dataset. This dataset should contain many images with hands. Notably, each hand in these images must be annotated, not only with its bounding box but also with its classification label denoting whether it is a non-standard hand or a standard hand. The dataset forms the bedrock of our methodology. 

\begin{figure}[!h]
    \centering
    \includegraphics[width=1\textwidth]{images/hagrid.png}
    \caption{HaGRID dataset samples and samples with bounding boxes.}
    \label{fig:hagrid}
\end{figure}

First, we use a large image dataset HaGRID (HAnd Gesture Recognition Image Dataset) \cite{hagrid} as our foundation. This dataset contains 552,992 FullHD RGB images showcasing hands in various postures. Each image within HaGRID comes meticulously annotated with bounding boxes, pinpointing the exact location of hands. The dataset encapsulates a diverse range of 18 unique hand gestures, performed by an ensemble of 34,730 distinct individuals ranging in age from 18 to 65. Some show one hand, some show both. The imagery was captured indoors under varying lighting conditions, ensuring a rich tapestry of visual nuances. Such diversity not only endows our dataset with broad coverage but also offers a commendable level of generalization, ensuring our model's robustness in handling hands across a vast spectrum of appearances. HaGRID dataset samples and samples with bounding box is illustrated in \autoref{fig:hagrid}.

\begin{figure}[h]
    \centering
    \includegraphics[width=1\textwidth]{images/redrawn.png}
    \caption{Redrawn samples by Stable Diffusion.}
    \label{fig:redrawn}
\end{figure}

We initiated our process by randomly selecting 30,000 images from the HaGRID dataset. Because these are real photos, all hands depicted in this subset are considered as standard hand. To generate corresponding transformed images, we use the Stable Diffusion \cite{2022_ldm} model to redraw the hand regions as delineated by their bounding boxes in the HaGRID images, their bounding boxes is provided in HaGRID dataset. As a result, for each \textit{Original} image from HaGRID, we now had a paired \textit{Redrawn} image. Redrawn samples is illustrated in \autoref{fig:redrawn}.

Due to inherent limitations in the Stable Diffusion model, a fraction of hands in the redrawn images manifested as non-standard hand. We manually selected some images from redrawn images containing non-standard hand, and forms a pair with its corresponding original image, the original image is standard hand. Each image in this set was annotated with labels and bounding boxes to indicate the presence and location of the hands. Subsequently, we partitioned the data into training and testing sets to ensure a robust evaluation of our model's performance. This is our dataset for detecting.

\subsection{Object Detection and Classification Model}

YOLOv8 \cite{yolov8} is a state-of-the-art model for object detection, instance segmentation, image classification, and pose estimation. To locate the hand and classify as non-standard hand or standard hand, we use training set mentioned above to fine-tune the YOLOv8 model. 

\begin{figure}[!h]
    \centering
    \includegraphics[width=1\textwidth]{images/bbox.png}
    \caption{Original samples with detected bounding box, redrawn samples with detected bounding box and redrawn samples with bounding box mask.}
    \label{fig:bbox}
\end{figure}

Upon deploying the trained YOLO model, the bounding boxes of hands are annotated, and the hands are classified accordingly. Only the non-standard hands are retained for restoration. The bounding boxes of these hands are converted into masks, which we refer to as bounding box mask. For a clearer understanding, we provide visual illustration in \autoref{fig:bbox}. All samples are selected from test set. From illustration we can know that fine-tuned model can correctly locate and classify the hand.

\section{Body Pose Estimation}

\begin{figure}[!h]
    \centering
    \includegraphics[width=1\textwidth]{images/mediapipe.png}
    \caption{Redrawn samples with body skeleton detected by MediaPipe.}
    \label{fig:mediapipe}
\end{figure}

To determine the size, position, and chirality of hands within our images, it is pivotal to estimate the body pose. \textit{MediaPipe} \cite{mediapipe}, a machine learning framework developed by Google, offers a plethora of solutions tailored for different vision-related tasks. Particularly, the \textit{Pose Landmark Detection} solution within MediaPipe can detect human body skeleton. It employs a machine learning model adept at pinpointing body landmarks in images or videos, such as hands, elbows, shoulders, hips, and more, along with the structural connections among them, as illustrated in \autoref{fig:mediapipe}.

\textit{Pose Landmark Detection} of MediaPipe distinguishes itself by offering three distinct landmarks for the hand is illustrated in \autoref{fig:hand_skeleton}, these landmarks subsequently act as instrumental cues, assisting us in ascertaining the hand's size, position, and gesture chirality. In contrast, other 2D pose estimation models \cite{alphapose, xu2022vitpose} extend only up to the wrist. In addition, this comprehensive body skeleton detection, even in cases where the hand imagery in non-standard hand images appears blurred or indistinct, ensures a certain level of prediction reliability.




\begin{figure}[!h]
	\centering
	\subfigure[Hand skeleton.]{
		\begin{minipage}[b]{0.40\textwidth}
			\includegraphics[height=6cm,keepaspectratio]{images/hand_skeleton.png} 
		\end{minipage}
		\label{fig:hand_skeleton}
	}
    \subfigure[Template: opened-palm.]{
		\begin{minipage}[b]{0.40\textwidth}
			\includegraphics[height=6cm,keepaspectratio]{images/template-a.png} 
		\end{minipage}
		\label{fig:template-a}
	}
 
	\subfigure[Template: fist-back.]{
		\begin{minipage}[b]{0.40\textwidth}
			\includegraphics[height=6cm,keepaspectratio]{images/template-b.png} 
		\end{minipage}
		\label{fig:template-b}
	}
    \subfigure[Template with landmark.]{
        \begin{minipage}[b]{0.40\textwidth}
        \includegraphics[height=6cm,keepaspectratio]{images/template_skeleton.png}
        \end{minipage}
    \label{fig:template_skeleton}
    }
    \caption{Hand and template details.}

\end{figure}

Upon detection, the skeletal landmarks were superimposed onto the redrawn image. For a more illustrative representation, the hand region were extracted and showcased in \autoref{fig:hand_skeleton}. The hand presents four salient landmarks: $a$, $b$, $c$, and $d$. Defining two vectors, $v_1 = \overrightarrow{ac}$ and $v_2 = \overrightarrow{bd}$, we compute their cross product $v_1 \times v_2$. The sign of the resultant aids in the classification of the hand orientation. If the result is negative, the hand is classified as a \textit{CW hand} (indicating a clockwise rotation from $v_1$ to $v_2$). Conversely, a positive result classifies the hand as a \textit{CCW hand} (signifying a counter-clockwise rotation from $v_1$ to $v_2$). This methodological classification offers us a straightforward approach to discern the chirality of the hand.


\section{Control Image Generation}

\begin{figure}[!h]
	\centering
	\subfigure[Background.]{
		\begin{minipage}[b]{0.3\textwidth}
			\includegraphics[height=5cm,keepaspectratio]{images/background.png} 
		\end{minipage}
		\label{fig:background}
	}
    \subfigure[Template in background.]{
		\begin{minipage}[b]{0.3\textwidth}
			\includegraphics[height=5cm,keepaspectratio]{images/template-in-background.png} 
		\end{minipage}
		\label{fig:template-in-background}
	}
	\subfigure[Template mask in background.]{
		\begin{minipage}[b]{0.3\textwidth}
			\includegraphics[height=5cm,keepaspectratio]{images/template-mask-in-background.png} 
		\end{minipage}
		\label{fig:template-mask-in-background}
    }
    \caption{Background, template in background and template mask in background.}
\end{figure}

\begin{figure}[!h]
	\centering
    \subfigure[Control image of redrawn samples.]{
		\begin{minipage}[b]{1\textwidth}
			\includegraphics[height=5cm,keepaspectratio]{images/control-c.png} 
		\end{minipage}
		\label{fig:control-image}
	}

    \subfigure[Union mask of redrawn samples.]{
		\begin{minipage}[b]{1\textwidth}
			\includegraphics[height=5cm,keepaspectratio]{images/control-e.png} 
		\end{minipage}
		\label{fig:union-mask}
	}

    \subfigure[Visualization of redrawn samples, body skeleton, control image and union mask.]{
		\begin{minipage}[b]{1\textwidth}
			\includegraphics[height=5cm,keepaspectratio]{images/control-a.png} 
		\end{minipage}
		\label{fig:visualization}
	}
    \caption{Some samples in control image generation.}
\end{figure}

\textit{ControlNet} \cite{2023_controlnet} has emerged as an enhancement to the \textit{Stable Diffusion} model. By incorporating additional input modalities, such as key landmarks, depth maps, edge maps, among others, \textit{ControlNet} steers \textit{Stable Diffusion} towards generating images with a more stable and realistic composition. This is important when aiming to restore hand representations in images, ensuring that the resultant shape, size, and contours adhere closely to real-world standards.

To optimize this restoration process, we engineer a \textit{ControlNet Image} as supplementary conditioning input. This image is specifically designed to assist \textit{Stable Diffusion} in effectively restoring the non-standard hands, pushing the boundaries of the model's capabilities and elevating the quality of the generated output. They are \textit{opened-palm} showed in \autoref{fig:template-a} and \textit{fist-back} showed in \autoref{fig:template-b}, which we refer to as \textit{Template}. It is easy to add more templates. An integral step involves meticulously positioning these Templates at precise hand locations to serve as the Control Image. The precision of this placement is paramount as it directly influences the \textit{ControlNet}'s ability to generate an accurate hand representation. To achieve this, we employ the following methodology:

\begin{enumerate}
    \item Similar to the hand landmarks detected via \textit{MediaPipe}, we manually annotate four specific points ($a'$, $b'$, $c'$, $d'$) on the Templates, as demonstrated in \autoref{fig:template_skeleton}. This allows us to construct vectors $v_1' = \overrightarrow{a'c'}$ and $v_2' = \overrightarrow{b'd'}$.
    
    \item Depending on the gesture and context of the image to be restored, an appropriate Template is chosen.
    
    \item We craft a \textit{background} image of identical dimensions to the redrawn image but entirely in black, as shown in \autoref{fig:background}. The whole Template image is then positioned at the top-left corner of the \textit{background}, is illustrated in \autoref{fig:template-in-background}. Concurrently, a white image of dimensions matching the Template, termed the \textit{template mask}, is placed at the top-left of the \textit{background}, is illustrated in \autoref{fig:template-mask-in-background}.
    
    \item The chirality of hand (CW hand or CCW hand) is first determined. If the hand chirality (CW hand or CCW hand) does not match the Template's chirality, the template is flipped to change its chirality.
    
    \item \textbf{Scaling}: The Template and the template mask are scaled by $\frac{|v_1|}{|v_1'|}$.
    
    \item \textbf{Moving}: The Template and the template mask are moved by $v_1 - v_1'$.
    
    \item \textbf{Rotation}: The Template and the template mask are rotated by $\theta$ degrees. If $a \times c' - c \times a' > 0$, we will rotate the Template clockwise, otherwise counterclockwise.
    
    $$\theta = \arccos{\frac{a a' + c c'}{\sqrt{a^2+c^2}\sqrt{a'^2+c'^2}}}$$
    
    \item The resultant image featuring the Template is coined as the \textit{control image}, as visualized in \autoref{fig:control-image}.

    \item The combined image of the template mask and the bounding box mask produces the \textit{union mask}, depicted in \autoref{fig:union-mask}.
    
    \item To offer a more comprehensive and intuitive perspective of the entire procedure, we have amalgamated samples of the redrawn images, body skeleton, control image, and union mask into a singular visual representation, as delineated in \autoref{fig:visualization}.
    
\end{enumerate}

It is necessary to use both YOLOv8 and MediaPipe results for this step, because MediaPipe can detect the occluded hand and cannot distinguish whether it is a non-standard hand, and YOLOv8 can compensate for this deficiency. By above methodology, we ensure that the Control Image provides the optimal cues to guide the \textit{ControlNet} in generating accurate hand reconstructions.


\section{ControlNet Inpainting}

\begin{figure}[!h]
    \centering
    \includegraphics[width=1\textwidth]{images/controlnet.png}
    \caption{ControlNet inpainting result.}
    \label{fig:controlnet}
\end{figure}

With the initial steps of delineating the hand's position and shape completed, we proceed to the task of image restoration using \textit{ControlNet}. This sophisticated restoration process hinges on the utility of the Union Mask to confine the areas of interest within the image, ensuring targeted and efficient improvements.

The \textit{Control Image}, with its adept location and representation of the hand, serves as an instructive guide for \textit{ControlNet} during the restoration of the redrawn image. To further refine and direct the restoration process, we complement this approach with a curated set of prompts. These prompts are meticulously chosen to invoke precise cues for the model, encapsulating the desired image attributes.

Our prompt is: ``\textit{[TEMPLATE NAME]}, hand, realskin, photorealistic, RAW photo, best quality, realistic, photo-realistic, masterpiece, an extremely delicate and beautiful, extremely detailed, 2k wallpaper, Amazing, finely detailed, 8k wallpaper, huge filesize, ultra-detailed, high-res, and extremely detailed.''

Additionally, we introduce a series of `negative prompts' to actively steer the model away from undesired outputs. These negative cues comprise: ``deformed, EasyNegative, paintings, sketches, (worst quality:2), (low quality:2), (normal quality:2), low-res, normal quality, and (monochrome).''

These keywords are commonly used by the community to gqenerate high-quality images and can be considered as part of the domain knowledge of prompt engineering.

By judiciously employing both the primary and negative prompts, we harness the prowess of \textit{ControlNet} to its full potential, ensuring the generation of images that are not only visually compelling but also adhere closely to real-world standards, is illustrated in \autoref{fig:controlnet}.


\section{IP2P Inpainting}

\begin{figure}[!h]
    \centering
    \includegraphics[width=1\textwidth]{images/ip2p.png}
    \caption{IP2P inpainting result.}
    \label{fig:ip2p}
\end{figure}


In the concluding phase of our methodology, we employ the capabilities of the \textit{instruct-pixel-to-pixel} (IP2P) model \cite{brooks2022instructpix2pix}. After achieving the preliminary restoration using \textit{ControlNet}, IP2P serves as an instrumental final touch, focusing primarily on texture enhancement. The essence of this phase is to impart a more life-like and authentic texture to the hands, ensuring their appearance seamlessly integrates with the rest of the image.

% 训练部分
First, we need the fine tune IP2P model. We use the training set in our dataset. The training set has 9623 pairs of images, and in each pair, there is a real image with standard hand selected from the HaGRID dataset, and a stable diffusion redraw image with non-standard hand.The real images served as input during training, while the redrawn images, with the non-standard hands, were utilized as the corresponding output. Alongside this, a Prompt, ``Turn the deformed hand into normal” and its 50 variants in \autoref{chap:appendix1}, were concurrently fed into training as input. This fine-tuning in an IP2P model adept at transforming non-standard hands into standard hand with heightened precision.

Then, We use the fine tuned model for restore. Contrasting with our previous steps, we refrain from using any masking at this juncture. The entirety of the image is processed, aligning the hand's texture and style with the global aesthetic of the picture. This holistic approach is facilitated using the directive prompt: ``Turn the deformed hand into normal''. 

The fruits of this step are illustrated in \autoref{fig:ip2p}, it is the final result of our restoration.


==> O-4-experiment.tex <==
\chapter{Experiment}\label{chap:experiment}

In the experiment chapter of this report, we will introduce the hardware and software configurations in \autoref{section:hardware_and_software} of the experiment, which is to ensure the reproducibility of the experimental results. Then we introduce the experimental procedures and results of detection and classification in \autoref{section:detection_and_classification} and restoration in \autoref{section:restoration} in detail. We then describe the experimental procedure and results of Detection and Classification and Restoration in detail, to demonstrate the validity of our methodology.

\section{Hardware and Software}\label{section:hardware_and_software}

For our experiments, we employed the following hardware and software setup:

\paragraph{Hardware:}
\begin{itemize}
    \item CPU: Intel Core i7-11700K
    \item GPU: NVIDIA GeForce RTX 3090
    \item Memory: 64GB RAM
\end{itemize}

\paragraph{Operating System and Drivers:}
\begin{itemize}
    \item OS: Ubuntu 22.04.3 LTS
    \item GPU Driver: NVIDIA Driver Version 535.113.01
    \item CUDA Version: 12.2
\end{itemize}

\paragraph{Software and Libraries:}
\begin{itemize}
    \item \textbf{Languages and Environments:} Python 3.11.4, conda 23.7.4.
    \item \textbf{Python Libraries of Deep Learning:} torch 2.0.1, torchvision 0.15.2, accelerate 0.23.0, transformers 4.33.2, ultralytics 8.0.180, timm 0.9.7, mediapipe 0.10.5
    \item \textbf{Python Libraries ofImage Processing:} Pillow 9.4.0, opencv-python 4.8.0.76
    \item \textbf{Python Libraries of Utilities and Others:} numpy 1.26.0, tqdm 4.65.0, gradio 3.44.3, matplotlib 3.8.0
\end{itemize}


\section{Detection and Classification}\label{section:detection_and_classification}

After manual selection from the redrawn images mentioned in \ref{section:method_detecting_database}, we identified 10,626 images, cumulatively containing 11,061 instances of Non-Standard Hands. This provided us with a paired dataset comprising 10,030 sets of images (an ``original" and its corresponding ``hand-redrawn" version). Each hand within these images is meticulously annotated with a bounding box and labeled either as a Non-Standard Hand or a Standard Hand. We use $0$ to represent the standard Hand, and $1$ to represent the non-standard hand. To facilitate both the training and evaluation phases, we partitioned our dataset: 90\% of the image pairs were allocated to the training set (9623 pairs images), while the remaining 10\% were reserved for the test set (1003 pairs images). We also counted the number of label, size and location of the bounding box  in the training set, which are shown in \autoref{fig:yolo_labels}.

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.7\textwidth]{images/yolo_labels.jpg}
    \caption{Number of label, size and location of the bounding box  in the training set}
    \label{fig:yolo_labels}
\end{figure}

Initially, we utilized the train set described in Section  to fine-tune the YOLOv8 model. Our training process commenced with the pretrained YOLOv8x model as the starting point, ensuring the model benefits from previously learned features while adapting to the nuances of our specific dataset. 

\paragraph{Some Training Parameters:}
\begin{itemize}
    \item Epochs: 100
    \item Batch Size: 96
    \item Automatic Mixed Precision (AMP): True
    \item Optimizer: Adam
    \item Dropout Rate: 0.0
\end{itemize}

\begin{figure}[!h]
    \centering
    \includegraphics[width=1\textwidth]{images/yolo_results.png}
    \caption{YOLOv8 train loss, test loss and metrics}
    \label{fig:yolo_results}
\end{figure}

The training spanned across 100 epochs, with a validation assessment performed at the end of each epoch. ~\autoref{fig:yolo_results} illustrates the progression of various metrics across epochs, encompassing train loss components (\textit{box\_loss}, \textit{cls\_loss}, \textit{dfl\_loss}), validation loss components (\textit{box\_loss}, \textit{cls\_loss}, \textit{dfl\_loss}) and metrics (\textit{precision}, \textit{recall}, \textit{mAP50}, and \textit{mAP50-95}). A noteworthy observation from the graph is the consistent decline in train and validation losses, with the latter stabilizing or showing a slight increment at certain epochs. Simultaneously, metrics like \textit{mAP50}, \textit{mAP50-95}, \textit{recall}, and \textit{precision} displayed an upward trend, stabilizing after certain epochs, underlining the efficacy and robustness of our training regimen.

\begin{table}[ht]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Class} & \textbf{Box Precision} & \textbf{Box Recall} & \textbf{mAP50} & \textbf{mAP50-95} \\
\hline
all & 0.904 & 0.933 & 0.971 & 0.888 \\
\hline
Standard Hand & 0.893 & 0.922 & 0.969 & 0.844 \\
\hline
Non-Standard Hand & 0.914 & 0.944 & 0.972 & 0.931 \\
\hline
\end{tabular}
\caption{Detection Results on Validation Set}
\label{tab:results}
\end{table}

Finally, we select the epoch with the best performance on the test set. The decision to capture the model's performance at its peak validation epoch enables us to circumvent overfitting and ensures the deployment of a stable model. \autoref{tab:results} summarizes the detection metrics of the model at its peak validation performance. Confusion matrices are illustrated in \autoref{fig:yolo_confusion_matrix}. To present a comprehensive view of our model's performance on the test set, we provide visual illustrations of various evaluation curves. \autoref{fig:yolo_curves} showcases the plotted metrics including the \textit{Precision curve}, \textit{Recall curve}, \textit{Precision-Recall}, and the \textit{F1 score curve}. These curves are paramount in understanding the trade-offs and overall effectiveness of our detection mechanism under different thresholds and conditions.

\begin{figure}[!h]
    \centering
    \includegraphics[width=1\textwidth]{images/yolo_confusion_matrix.png}
    \caption{Confusion matrices}
    \label{fig:yolo_confusion_matrix}
\end{figure}

\begin{figure}[!h]
	\centering
    \centering
    \includegraphics[width=1\textwidth]{images/yolo_curves.png}
    \caption{Precision, Recall, Precision-Recall, F1 score}
    \label{fig:yolo_curves}

\end{figure}


Through our extensive experiments, it became evident that the accuracy of bounding box placement significantly influences the restoration quality. A slight misalignment or offset in the bounding box can drastically deteriorate the subsequent rectification results. As such, relying solely on commonly adopted metrics like IOU (Intersection over Union) with a threshold of 50\% (e.g., mAP50) is inadequate for our specific application.

In our context, achieving higher precision in bounding box placement is pivotal, necessitating the exploration of stricter IOU thresholds, such as 80\% and above. Moreover, we prioritize a high recall rate in our evaluations. Our rationale is that while erroneously rectifying a \textit{Standard Hand} is undesirable, the oversight of a \textit{Non-Standard Hand} is even more detrimental and less acceptable.

To this end, we conducted evaluations across various IOU thresholds to understand their implications on the detection outcomes.

\begin{table}[!h]
\centering
\caption{Detection Outcomes across Different IOU Thresholds}
\label{tab:IOU_results}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{IOU Threshold} & \textbf{TP} & \textbf{FP} & \textbf{FN} & \textbf{TN} & \textbf{Precision} & \textbf{Recall} \\
\hline
0.80 & 1019 & 132 & 185 & 988 & 0.89 & 0.85 \\
\hline
0.85 & 994 & 157 & 246 & 927 & 0.86 & 0.86 \\
\hline
0.90 & 936 & 215 & 443 & 730 & 0.81 & 0.68 \\
\hline
0.95 & 721 & 430 & 930 & 243 & 0.63 & 0.44 \\
\hline
\end{tabular}
\end{table}

As discerned from Table~\ref{tab:IOU_results}, the model achieves a commendable \textit{Precision} of 0.89 and \textit {Recall} of 0.85 when the IOU threshold is set at a stringent criterion of 0.80. Furthermore, when considering the mAP at 50\% IOU (mAP50), our model impressively reaches a score of 0.971. These metrics corroborate the assertion that our fine-tuned YOLO model exhibits robust and precise detection capabilities on the test set. The exceptional performance, especially at higher IOU thresholds, underscores its proficiency in accurately delineating and recognizing target objects. 

% \section{IP2P model}

\section{Restoration} \label{section:restoration}

\subsection{Evaluation Metric: Fréchet Inception Distance (FID)}
To evaluate the quality of our restored images, we employed the Fréchet Inception Distance (FID). The FID metric assesses the quality of images produced by a generative model. FID makes a comparative assessment by juxtaposing the distribution of the generated images against that of a set of real images, or what is commonly referred to as "ground truth". The primary essence of FID is to compute the distance between feature vectors of the real and generated images. A smaller FID value indicates a higher degree of similarity between the distributions. Ideally, an FID value of 0 signifies perfect similarity, implying that the two images under comparison are identical.

\subsection{Restoration Results}

Our image restoration process primarily focused on images bearing non-standard hands, which were regenerated using the Stable Diffusion process. The originating dataset, HaGRID, originally contained images with standard hands. Our assessment phase involved comparisons of various image sets: the original images with standard hands, images with non-standard hands, ControlNet inpainting results, and IP2P inpainting results. The outcomes of these evaluations are summarized in Table 1.

A critical observation from \autoref{table:fid} is that the FID score between images with standard hands and images with non-standard hands is the highest. This underscores the apparent disparity between the original and redrawn images. Conversely, the comparison between images with standard hands and the ControlNet inpainting results yields a slightly better FID score, signifying moderate restoration effectiveness. Notably, the most promising results are observed when comparing the IP2P inpainting results, showcasing the lowest FID score. This accentuates the efficacy of our restoration process, with IP2P inpainting offering superior results, more closely approximating the standard hand images and thus effectively restoring the non-standard hands.


\begin{table}[!h]
\begin{tabular}{ll}
\hline
\textbf{FID with standard hand} & \textbf{FID} \\ \hline
Non-standard hand               & 52.92        \\
ControlNet inpainting           & 41.19        \\
IP2P inpainting                 & 33.23        \\ \hline
\end{tabular}
\caption{FID comparing different image sets for hand restoration.}
\label{table:fid}
\end{table}

In addition, we have conducted experiments on various styles of pictures with non-standard hand to check the generalization ability of our model. As demonstrated in \autoref{fig:multi-style}, the model's performance is consistently reliable across different sources of images. This includes images redrawn from HaGRID \cite{hagrid}, redrawn from real photos, and images generated by the Stable Diffusion \cite{2022_ldm} model. These results show that the model is effective for different styles of images, can fix their non-standard hand, and the model has good generalization performance.

\begin{figure}[!h]
    \centering
    \includegraphics[width=1\textwidth]{images/experiment/multi-style-ps.png}
    \caption{Various styles of pictures with non-standard hand.}
    \label{fig:multi-style}
\end{figure}

% In the context of our research, an initial inclination was to harness GSA as the primary mechanism for hand detection, encompassing both standard and non-standard hand depictions. However, as exploratory evaluations unfurled, we discerned some limitations in GSA's capability. Specifically, the model exhibited challenges in differentiating between standard and non-standard hand representations. When instructed to detect "standard hand", GSA would indiscriminately return all hand images. Sometimes extending its segmentation to include entire arms in non-standard hands. Due to these inconsistencies and the model's inability to make nuanced distinctions, we eventually opted not to incorporate GSA in our finalized approach.




==> O-5-software.tex <==
\chapter{Software}\label{chap:software}

\section{Overview and Getting Started}

The main goal of our project is to improve the human generation capability of stable diffusion, so making it fast and easy for users to use is our fundamental goal. So software is one of the most important parts of our project, its screenshot is showed in \autoref{screenshot}. We introduce a user-friendly web application based on the \textit{Gradio} framework. This application serves as an interactive portal allowing users to input images containing non-standard hands and promptly receive the rectified results. Our web application enables users to interact directly via a browser on devices lacking GPU support, such as mobile devices. This browser-based approach eliminates the intricacies of deploying a Python program, making it especially accessible for non-experts. Designed with a step-by-step approach, it not only aids users in comprehending the restoration process but also offers flexibility in parameter adjustments during the restoration process. To get started, simply navigate to \url{http://gradio.yiqun.io} in your browser.

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.8\textwidth]{images/software/screenshot-1.png}
    \caption{Screenshot of a part of the webapp.}
    \label{fig:screenshot}
\end{figure}

\section{Non-Standard Hand Detection}

This phase focuses on the identification of hands present within the provided image, further classifying them as either non-standard or standard hands. Once the non-standard hands are detected, they are represented as masks, facilitating the subsequent restoration process.

\subsection{Inputs and Parameters}

As shown in \autoref{fig:s1-input}, this step incorporates a primary input and two adjustable parameters:

\begin{itemize}
    \item \textbf{Original Image}: By default, a sample image containing a non-standard hand is preloaded to offer users an immediate experience of our web application. If desired, this sample image can be cleared by clicking the upper right `X', allowing users to upload a new image.
    \item \textbf{Bounding Box Mask Include Standard Hand}: This checkbox, when activated, instructs the application to restore not just the non-standard hands but all detected hands, encompassing both non-standard and standard ones.
    \item \textbf{Bounding Box Mask Expand Ratio}: This slider allows users to adjust the size of the detected bounding box. For those seeking a more precise restoration outcome, this parameter can be manually fine-tuned.
\end{itemize}

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.6\textwidth]{images/software/s1-input.png}
    \caption{Inputs and Parameters of Step 1.}
    \label{fig:s1-input}
\end{figure}

\subsection{Outputs}

Following the detection and categorization process, three primary outputs are generated, as depicted in \autoref{fig:s1-output}:

\begin{itemize}
    \item \textbf{Number of Hands \& Classification with Confidence}: This display enumerates the detected hands and categorizes them as either `standard hand' or `non-standard hand', accompanied by a confidence score for each classification.
    \item \textbf{Bounding Box}: The detected hands are visually represented with bounding boxes. Non-standard hands are encircled in red, while standard hands are highlighted in green.
    \item \textbf{Bounding Box Mask}: This output represents the non-standard hands as masks, to future restoration process.
\end{itemize}

\begin{figure}[!h]
    \centering
    \includegraphics[width=1\textwidth]{images/software/s1-output.png}
    \caption{Outputs of Step 1.}
    \label{fig:s1-output}
\end{figure}

\section{Body Pose Estimation}

The primary objective of this phase is to conduct a comprehensive Body Pose Estimation. The main emphasis is on acquiring the skeleton of both the body and the hand, ensuring a precise determination of the hand's position and orientation. Such insights are pivotal for achieving superior restoration results in the subsequent stages.

\subsection{Inputs and Parameters}

This step does not demand any additional inputs from the user. Instead, it utilizes the original image provided during the previous non-standard hand detection phase.

\subsection{Outputs}

Upon completion of the body pose estimation, two outputs are generated, as showcased in \autoref{fig:s2-output}:

\begin{itemize}
    \item \textbf{Key Points String}: This display enumerates the detected body landmarks, providing users with a detailed insight into the specific skeletal keypoints identified.
    \item \textbf{Body Skeleton Visualization}: Building on the aforementioned keypoints, this output draws connections between them directly onto the original image. This offers users a clear, visual representation of the body's structural orientation and the relative positioning of the hands.
\end{itemize}


\begin{figure}[!h]
    \centering
    \includegraphics[width=0.6\textwidth]{images/software/s2-output.png}
    \caption{Outputs of Step 2.}
    \label{fig:s2-output}
\end{figure}

\section{Control Image Generation}

During this phase, the objective is to produce a Control Image. The Control Image serves to guide the control map. In this step, a hand template is positioned onto the detected hand location. This placement defines the hand's shape, size, and orientation, establishing the parameters crucial for the upcoming restoration process.

\subsection{Inputs and Parameters}

There is no need for fresh input at this stage; the process leans on the results from previous phases. Three essential parameters come into play as depicted in \autoref{fig:s3-input}:

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.7\textwidth]{images/software/s3-input.png}
    \caption{Inputs of Step 3.}
    \label{fig:s3-input}
\end{figure}

\begin{itemize}
    \item \textbf{Hand Template}: Users have the liberty to select from various hand templates. Currently, there are two templates available: opened-palm and fist-back, as displayed in \autoref{fig:s3-template}. Developers can further extend this list by adding templates as per specific requirements.
    \item \textbf{Control Image and Mask Expand Ratio (From Wrist)}: This slider grants users the ability to resize the selected hand template. For those seeking heightened precision in their restoration results, fine-tuning this parameter is advisable.
    \item \textbf{Include Undetected Hand}: Activating this checkbox ensures the restoration of hands which were undetected during the non-standard hand detection phase but were predicted during the body pose estimation phase. Typically, altering this option isn't recommended.
\end{itemize}

\begin{figure}[!h]
	\centering
	\subfigure[Opened-palm.]{
		\begin{minipage}[b]{0.45\textwidth}
			\includegraphics[height=5cm,keepaspectratio]{images/software/template-a.png} 
		\end{minipage}
	}
    \subfigure[Fist-back.]{
		\begin{minipage}[b]{0.45\textwidth}
			\includegraphics[height=5cm,keepaspectratio]{images/software/template-b.png} 
		\end{minipage}
	}

    \caption{Hand Templates.}
    \label{fig:s3-template}
\end{figure}

\subsection{Outputs}

Post-execution of this phase, five outputs are generated as shown in \autoref{fig:s3-output}:

\begin{itemize}
    \item \textbf{Visualization Image}: Provides a composite view, integrating the Original Image, Control Mask, bounding box mask, Body Skeleton, and Control Image into a single frame. This visual aid allows users to grasp the progression of the restoration.
    \item \textbf{Combine Image}: Merges the Control Image with the Original Image, letting users observe the accuracy in positioning, size, and orientation of the template.
    \item \textbf{Control Image}: This output showcases the template accurately placed onto its intended location.
    \item \textbf{Control Mask}: Outlines the template, functioning akin to the bounding box mask by constraining the area for the subsequent inpainting process.
    \item \textbf{Union Mask}: This mask is the result of amalgamating the Control Mask with the earlier generated bounding box mask, further demarcating the region designated for restoration.
\end{itemize}


\begin{figure}[!h]
    \centering
    \includegraphics[width=1\textwidth]{images/software/s3-output.jpg}
    \caption{Outputs of Step 3.}
    \label{fig:s3-output}
\end{figure}


\section{ControlNet Inpainting}

This phase harnesses the capabilities of ControlNet for inpainting purposes, focusing specifically within the boundaries delineated by the previously generated union mask.

\subsection{Inputs and Parameters}

In this step, no additional input is required, nor are there any parameters to adjust. Should the outcome generated by this step be unsatisfactory, users are encouraged to resubmit for potential enhancements.

\subsection{Outputs}

Upon completing this stage, one key output is generated, as illustrated in \autoref{fig:s4-output}: the result of the ControlNet Inpainting process. This visualization aids users in understanding the improvements made by the ControlNet algorithm on the original image.


\begin{figure}[!h]
    \centering
    \includegraphics[width=0.6\textwidth]{images/software/s4-output.png}
    \caption{Outputs of Step 4.}
    \label{fig:s4-output}
\end{figure}


\section{IP2P Inpainting}

During this phase, inpainting is executed via the IP2P approach, targeting the entirety of the image.

\subsection{Inputs and Parameters}

This step refrains from seeking any additional input and offers no parameters for customization. In the event that the result produced by this stage is not up to par, users can resubmit to strive for better outcomes.

\subsection{Outputs}

Consequent to the completion of this process, a singular output is presented, showcased in \autoref{fig:s5-output} the resultant image from the IP2P Inpainting procedure. This visual representation provides users with a comprehensive understanding of the refinements achieved by the IP2P methodology on the initial image. This is the final result of the restoration.


\begin{figure}[!h]
    \centering
    \includegraphics[width=0.6\textwidth]{images/software/s5-output.png}
    \caption{Outputs of Step 5.}
    \label{fig:s5-output}
\end{figure}


% \section{Privacy Measures}

==> O-6-conclusion.tex <==
\chapter{Concluding Remarks}\label{chap:conclusion}

\section{Conclusion}

In the landscape of computer vision, achieving realism in generative models is of utmost significance. One of the challenges faced by the Stable Diffusion model \cite{2022_ldm}, namely the generation of non-standard hand images, became the focal point of our research.

Through the deployment of our methodological approach, we observed promising outcomes. The detection phase, enhanced by the YOLO model \cite{yolov8}, proficiently identified the hand locations within images and categorized them into non-standard hand or standard hand. We used various indicators to comprehensively evaluate the test set consisting of 2006 images. These images cover a variety of scenes and gestures, and we use Precision and Recall of 0.85, 0.90, 0.95. Among these evaluation indicators, our models have achieved excellent notes. This comprehensive evaluation not only enhances the effectiveness of our detection method, but also emphasizes the robustness and versatility of our model in dealing with various real-world scenarios, which shows that the model can effectively detect non-standard images generated by Stable Diffusion. Hands.

The restoration phase of our pipeline further reinforced the results. Each step, from body pose estimation to control image generation and the subsequent inpainting processes, was meticulously designed to ensure the hands were not only accurately detected but also restored with precision. We have shown using FID that result of ControlNet inpainting is better than image with non-standard hand, and result of IP2P inpainting is better than result of ControlNet inpainting, and our ControlNet inpainting and IP2P inpainting are both valid. In addition to using redrawn samples from the HaGRID dataset, we have also experimented with images generated entirely by Stable Diffusion and real images, both of which yielded satisfactory restoration results. Our experiments show that our methodology consistently transformed the non-standard hand images closer to their standard hand counterparts.

In summary, our research contributes a significant step forward in enhancing the Stable Diffusion model, especially concerning hand representation in generated images. The experiments conducted across various datasets provided concrete evidence of the effectiveness and versatility of our proposed approach.


\section{Future Work}

\paragraph{Complex Hand Interactions:} Our current methodology relies on an accurate 2D hand template placement, which poses challenges in situations where two hands are intricately interwoven. This limitation underscores the intricacy of hands as 3D structures. Subtle 3D alterations, such as rotations, can introduce significant variations in the 2D projection, often losing nuances like depth, orientation, and precise positioning. An intriguing avenue for future investigation might be the incorporation of 3D models and understandings to alleviate some challenges in 2D AI Generated Content.

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.7\textwidth]{images/bad.png}
    \caption{Intricately interwoven.}
    \label{fig:bad}
\end{figure}


\paragraph{Expansion to Other Body Parts:} 

While our research primarily focuses on hand image generation and rectification, the proposed framework could be extended to address other body parts, ensuring a more holistic and coherent image generation and rectification process.

\paragraph{Integration with Advanced AI Painting Models:} To elevate the overall quality of generated images, future work can explore the integration of our method with more advanced AI painting models. Such synergies could potentially address broader image imperfections beyond just hands.

\paragraph{Advanced Body Pose Estimation:} While MediaPipe serves as our current body pose estimation model, it is not the state-of-the-art. The renowned ViT-Pose \cite{xu2022vitpose} offers superior performance. However, its limited scope (detection up to the wrist without detailed hand landmarks) makes it unsuitable for our needs. Future endeavors will use better skeletal detection methods, aiming to achieve a more accurate restoration process. For example, we can modify and retrain ViT-Pose so that it can predict the keypoints in the hand.


% Low resolution

==> diff_model_foundation.tex <==
\subsection{Foundations of Diffusion Models}

Diffusion models represent a class of probabilistic generative paradigms that iteratively modulate data through the infusion of noise, subsequently mastering the inversion of this process for the generation of samples. The core concept of diffusion models is elucidated in \autoref{fig:diffusion_schematic}. Recent investigations chiefly revolve around three seminal formulations: denoising diffusion probabilistic models (DDPMs)~\cite{sohl2015deep,ho2020denoising,nichol2021improved}, score-based generative models (SGMs)~\cite{song2019generative,song2020improved}, and stochastic differential equations cast as Score SDEs~\cite{song2020score,song2021maximum}. In this exposition, we delineate the denoising diffusion probabilistic models. 

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{images/diffusion_schematic.png}
    \caption{Diffusion models infuse noise into data, thereafter retracing this process to foster new data from noise. Each denoising step in the reversionary journey necessitates the estimation of the score function (refer to the illustrative figure on the right), a gradient suggestive of the data directions emblematic of augmented likelihood and attenuated noise. \label{fig:diffusion_schematic}}
\end{figure*}

A \emph{denoising diffusion probabilistic model} (DDPM) \cite{sohl2015deep,ho2020denoising} utilizes two Markov chains: a forward one that morphs data into noise, and a reverse one that restores noise back to data. The forward chain is traditionally designed with the aim of transitioning any data distribution into a simplified prior distribution (e.g., standard Gaussian), while the reverse chain strives to invert this transformation by learning transition kernels, which are parameterized by neural networks. The generation of new data points is accomplished by initially sampling a random vector from the prior distribution, which is then subjected to ancestral sampling through the reverse Markov chain~\cite{koller2009probabilistic}.

Formally, given a data distribution $\mathbf{x}_0 \sim q(\mathbf{x}_0)$, the forward Markov process engenders a sequence of random variables $\mathbf{x}_1, \mathbf{x}_2, \ldots, \mathbf{x}_T$, driven by the transition kernel $q(\mathbf{x}_t\mid\mathbf{x}_{t-1})$. Utilizing the chain rule of probability in conjunction with the Markov property, the joint distribution of $\mathbf{x}_1, \mathbf{x}_2, \ldots, \mathbf{x}_T$ conditioned on $\mathbf{x}_0$, denoted as $q(\mathbf{x}_1, \ldots, \mathbf{x}_T\mid\mathbf{x}_0)$, can be expounded as
\begin{align}
    q(\mathbf{x}_1, \ldots, \mathbf{x}_T\mid\mathbf{x}_0) &= \prod_{t=1}^{T} q(\mathbf{x}_t\mid\mathbf{x}_{t-1}).\label{eq:forward_joint}
\end{align}

In DDPMs, the transition kernel \(q(\mathbf{x}_t \mid \mathbf{x}_{t-1})\) is judiciously crafted to progressively transmute the data distribution \(q(\mathbf{x}_0)\) into a tractable prior distribution. A common design for the transition kernel encompasses Gaussian perturbation, with a prevalent choice being
\begin{align}
    q(\mathbf{x}_t\mid\mathbf{x}_{t-1}) &= \mathcal{N}(\mathbf{x}_t; \sqrt{1-\beta_t} \mathbf{x}_{t-1}, \beta_t \mathbf{I}), \label{eq:2}
\end{align}
where \(\beta_t \in (0,1)\) is a pre-specified hyperparameter prior to model training. This kernel is utilized to streamline our discussion herein, although alternative kernels can be employed analogously. As elucidated by Sohl-Dickstein et al. (2015) \cite{sohl2015deep}, this Gaussian transition kernel facilitates the marginalization of the joint distribution in~\autoref{eq:forward_joint}, rendering the analytical form of \(q(\mathbf{x}_t \mid \mathbf{x}_0)\) for all \(t \in \{0,1,\cdots,T\}\). Specifically, with \(\alpha_t \coloneqq 1 - \beta_t\) and \(\bar{\alpha}_t \coloneqq \prod_{s=0}^{t} \alpha_s\), we deduce
\begin{align}
        q(\mathbf{x}_t\mid\mathbf{x}_0) &= \mathcal{N}(\mathbf{x}_t; \sqrt{\bar{\alpha}_t} \mathbf{x}_0, (1-\bar{\alpha}_t) \mathbf{I}) \label{eq:3}.
\end{align}
Given \(\mathbf x_0\), a sample of \(\mathbf{x}_t\) can be effortlessly obtained by sampling a Gaussian vector \(\bepsilon \sim \mathcal{N}(\mathbf{0}, \mathbf{I})\) and applying the transformation
\begin{align}
    \mathbf{x}_t &=\sqrt{\bar{\alpha}_t} \mathbf{x}_0 + \sqrt{1-\bar{\alpha}_t} \bepsilon. \label{eq:4}
\end{align}
When \(\bar{\alpha}_T \approx 0 \), \(\mathbf{x}_{T}\) approximates a Gaussian distribution, thereby rendering \(q(\mathbf x_T) \coloneqq \int q(\mathbf x_T \mid \mathbf x_0) q(\mathbf x_0) \textrm{d} \mathbf x_0 \approx \mathcal{N}(\mathbf x_T; \mathbf{0}, \mathbf{I})\).

Intuitively, this forward process incrementally injects noise into the data until all inherent structures are obscured. To generate data samples, DDPMs commence by creating a noise vector from the prior distribution (which is generally straightforward to obtain), then progressively eliminate noise through the execution of a learnable Markov chain in the reverse temporal direction. Specifically, the reverse Markov chain is characterized by a prior distribution \(p(\mathbf x_T) = \mathcal{N}(\mathbf x_T; \mathbf{0}, \mathbf{I})\) and a learnable transition kernel \(p_\theta(\mathbf{x}_{t-1}\mid\mathbf{x}_t)\). The choice of prior distribution \(p(\mathbf x_T) = \mathcal{N}(\mathbf x_T; \mathbf 0, \mathbf I)\) is inspired by the construction of the forward process such that \(q(\mathbf x_T) \approx \mathcal{N}(\mathbf x_T; \mathbf{0}, \mathbf{I})\). The learnable transition kernel \(p_\theta(\mathbf{x}_{t-1}\mid\mathbf{x}_t)\) is articulated as
\begin{align}
  p_\theta(\mathbf x_{t-1}\mid\mathbf x_t) &= \mathcal{N}(\mathbf x_{t-1}; \mu_{\theta}(\mathbf x_t, t), \Sigma_{\theta}(\mathbf x_t, t))
  \label{4}
\end{align}
where \(\theta\) denotes model parameters, with the mean \(\mu_{\theta}(\mathbf x_t, t)\) and variance \(\Sigma_{\theta}(\mathbf x_t, t)\) being parameterized by neural networks. Equipped with this reverse Markov chain, a data sample \(\mathbf x_0\) can be generated by initially sampling a noise vector \(\mathbf x_T \sim p(\mathbf x_T)\), followed by iterative sampling from the learnable transition kernel \(\mathbf x_{t-1} \sim p_\theta(\mathbf x_{t-1} \mid \mathbf x_t)\) until \(t = 1\).

Central to the efficacy of the sampling process is the alignment training of the reverse Markov chain to mirror the actual time reversal of the forward Markov chain. This involves tuning the parameter \(\theta\) such that the joint distribution of the reverse Markov chain \(p_\theta(\mathbf x_0, \mathbf x_1, \cdots, \mathbf x_T)\coloneqq p(\mathbf x_T)\prod_{t=1}^T p_\theta(\mathbf x_{t-1}\mid\mathbf x_t)\) closely reflects that of the forward process \(q(\mathbf x_0, \mathbf x_1, \cdots, \mathbf x_T) \coloneqq q(\mathbf x_0) \prod_{t=1}^T q(\mathbf x_t \mid \mathbf x_{t-1})\) (\autoref{eq:forward_joint}). This alignment is implemented by minimizing the Kullback-Leibler (KL) divergence between the two distributions:
\begin{align}
    &\operatorname{KL}(q(\mathbf x_0, \mathbf x_1, \cdots, \mathbf x_T) \mid\mid p_\theta(\mathbf x_0, \mathbf x_1, \cdots, \mathbf x_T))\\
    \stackrel{(i)}{=} &-\mathbb{E}_{q(\mathbf x_0, \mathbf x_1, \cdots, \mathbf x_T)}[\log p_\theta(\mathbf x_0, \mathbf x_1, \cdots, \mathbf x_T)] + \text{const}\\
    \stackrel{(ii)}{=} & \underbrace{\mathbb{E}_{q(\mathbf x_0, \mathbf x_1, \cdots, \mathbf x_T)}\bigg[ -\log p(\mathbf x_T) - \sum_{t=1}^T \log \frac{p_\theta(\mathbf x_{t-1}\mid\mathbf x_t)}{q(\mathbf x_t\mid\mathbf x_{t-1})} \bigg]}_{\coloneqq -L_{\textrm{VLB}}(\mathbf x_0)} + \text{const} \label{eq:7} \\
    \stackrel{(iii)}{\geq} & \mathbb{E}_{- \log p_\theta(\mathbf x_0)} + \text{const},
\end{align}
where (i) stems from the definition of KL divergence, (ii) arises from the fact that \(q(\mathbf x_0, \mathbf x_1, \cdots, \mathbf x_T)\) and \(p_\theta(\mathbf x_0, \mathbf x_1, \cdots, \mathbf x_T)\) are both products of distributions, and (iii) follows from Jensen's inequality. The first term in \autoref{eq:7} denotes the variational lower bound (VLB) of the log-likelihood of the data \(\mathbf x_0\), a typical objective in training probabilistic generative models. The notation ``\(\text{const}\)'' represents a constant independent of the model parameter \(\theta\), and thus does not impact optimization. The goal of DDPM training is to increase the VLB (also equivalently, minimize the negative VLB). This objective is notably tractable for optimization given its formulation as a sum of independent terms, allowing for efficient estimation via Monte Carlo sampling~\cite{metropolis1949monte} and effective optimization through stochastic optimization techniques~\cite{spall2012stochastic}.

In a seminal work, Ho et al.~\cite{ho2020denoising} propose a re-weighting scheme for the distinct terms in \(L_\textrm{VLB}\) to ameliorate sample quality. They discern a notable correspondence between the resultant loss function and the training objective of noise-conditional score networks (NCSNs), a variant of \emph{score-based generative models}, as expounded by Song and Ermon~\cite{song2019generative}. The formulated loss in~\cite{ho2020denoising} is delineated as
\begin{align}
    \mathbb{E}_{t \sim \mathcal{U}\llbracket 1,T \rrbracket, \mathbf x_0 \sim q(\mathbf x_0), \bepsilon \sim \mathcal{N}(\mathbf{0},\mathbf{I})}{ \lambda(t)  \left\| \bepsilon - \bepsilon_\theta(\mathbf{x}_t, t) \right\|^2} \label{8}
\end{align}
where \(\lambda(t)\) denotes a positive weighting function. The variable \(\mathbf x_t\) is deduced from \(\mathbf x_0\) and \(\bepsilon\) as per \autoref{eq:4}. The term \(\mathcal{U}\llbracket 1, T \rrbracket\) signifies a uniform distribution over the set \(\{1, 2, \cdots, T\}\). Moreover, \(\bepsilon_{\theta}\) refers to a deep neural network with parameter \(\theta\), engineered to predict the noise vector \(\bepsilon\) given \(\mathbf{x}_{t}\) and \(t\). This objective transitions to \autoref{eq:7} with a particular choice for the weighting function \(\lambda(t)\), and bears resemblance to the loss function employed in denoising score matching across multiple noise levels for the training of score-based generative models~\cite{song2019generative}.


==> discussion.tex <==
\section{Discussion}

We conjecture that Stable Diffusion tends to generate non-standard hands because of its inherent challenges in capturing spatial positioning, proportions, and detailed intricacies, particularly in 3D to 2D representations. We draw insights from \cite{ramesh2022hierarchical}, DallE2, another diffusion model. It has also shown limitations in handling spatial positioning and proportions, as evident from \autoref{fig:intro-dalle-1}, one input (red cube on top, blue cube on bottom) gets a lot of confusing outputs. In addition, \autoref{fig:intro-dalle-2} shows the model's challenges in capturing intricate details within complex scenes. A significant contributor to this limitation might be the Contrastive Language-Image Pre-Training (CLIP) architecture they employed. In the CLIP training phase, the model predominantly learns from holistic image descriptions, often overlooking fine details such as those of hands. Thus, the nuances of hand articulations might elude these models. Another plausible explanation for this observed anomaly in hand generation could be the inherent complexity of hands as a 3D structure. Even slight alterations, such as rotations, can introduce significant variances when represented in a 2D image. Since Stable Diffusion primarily trains on 2D representations, it might be challenged in assimilating the comprehensive 3D intricacies of hands. This insufficiency potentially results in detailed inaccuracies when generating novel hand images.

\begin{figure}[!h]
    \centering
	\subfloat[Confused spatial positioning.]{
        \label{fig:intro-dalle-1}
        \includegraphics[width=0.45\linewidth]{images/introduction/dalle-1.png}
    }
	\subfloat[Complex scene.]{
        \label{fig:intro-dalle-2}
        \includegraphics[width=0.45\linewidth]{images/introduction/dalle-2.png}
    }

    \caption{Illustrations from \cite{ramesh2022hierarchical}.}
    \label{fig:intro-dalle} 
\end{figure}
